Comparing Star Formation on Large Scales in the c2d Legacy Clouds: Bolocam 1.1 mm Dust Continuum Surveys of Serpens, Perseus, and Ophiuchus

We have undertaken an unprecedentedly large 1.1 millimeter continuum survey of three nearby star forming clouds using Bolocam at the Caltech Submillimeter Observatory. We mapped the largest areas in each cloud at millimeter or submillimeter wavelengths to date: 7.5 sq. deg in Perseus (Paper I), 10.8 sq. deg in Ophiuchus (Paper II), and 1.5 sq. deg in Serpens with a resolution of 31", detecting 122, 44, and 35 cores, respectively. Here we report on results of the Serpens survey and compare the three clouds. Average measured angular core sizes and their dependence on resolution suggest that many of the observed sources are consistent with power-law density profiles. Tests of the effects of cloud distance reveal that linear resolution strongly affects measured source sizes and densities, but not the shape of the mass distribution. Core mass distribution slopes in Perseus and Ophiuchus (alpha=2.1+/-0.1 and alpha=2.1+/-0.3) are consistent with recent measurements of the stellar IMF, whereas the Serpens distribution is flatter (alpha=1.6+/-0.2). We also compare the relative mass distribution shapes to predictions from turbulent fragmentation simulations. Dense cores constitute less than 10% of the total cloud mass in all three clouds, consistent with other measurements of low star-formation efficiencies. Furthermore, most cores are found at high column densities; more than 75% of 1.1 mm cores are associated with Av>8 mag in Perseus, 15 mag in Serpens, and 20-23 mag in Ophiuchus.

==> tab1.tex <==
\ProvidesFile{tab1.tex}
\begin{deluxetable}{lcccccc}
\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{Sources Found in Serpens \label{srctab}}
\tablehead{
\colhead{ID} & \colhead{RA (2000)} & \colhead{Dec (2000)} & \colhead{Peak} &  \colhead{S/N}  & \colhead{other names} & \colhead{MIPS source?}  \\ 
 \colhead{} & \colhead{($h ~~m ~~s$)} & \colhead{($\degr~~ \arcmin~~ \arcsec$)} & \colhead{(mJy/beam)} &  \colhead{}  & \colhead{} & \colhead{}  
}
\startdata
Bolo1  &  18 28 23.1 &  +00 26 34.6  &  95 (12)  &  5.0  &    &  N   \\
Bolo2  &  18 28 44.0 &  +00 53 02.8  &  198 (12)  &  9.9  &    &  N   \\
Bolo3  &  18 28 45.8 &  +00 51 32.4  &  227 (12)  &  13.7  &  IRAS 18262+0050  &  Y   \\
Bolo4  &  18 28 47.2 &  +00 50 45.1  &  145 (10)  &  7.1  &    &  N  \\
Bolo5  &  18 28 48.3 &  +00 14 51.5  &  73 (9)  &  5.8    &    &  N   \\
Bolo6  &  18 28 50.8 &  +00 50 28.6  &  115 (10)  &  7.3  &    &  N   \\
Bolo7  &  18 28 53.0 &  +00 19 03.6  &  119 (11)  &  5.4  &    &  Y   \\
Bolo8  &  18 28 55.2 &  +00 29 28.0  &  617 (13)  &  30.8  &  IRAS 18263+0027; MMS1 (2)  &  Y   \\
Bolo9  &  18 28 55.9 &  +00 48 30.3  &  141 (10)  &  9.1  &    &  N   \\
Bolo10  &  18 28 56.6 &  +00 19 10.4  &  107 (11)  &  5.7  &    &  N   \\
Bolo11  &  18 28 57.3 &  +00 48 06.5  &  162 (11)  &  10.9  &    &  N   \\
Bolo12  &  18 28 58.4 &  +00 47 35.7  &  172 (11)  &  12.0  &    &  N   \\
Bolo13  &  18 29 00.2 &  +00 30 19.8  &  239 (15)  &  5.5  &    &  Y   \\
Bolo14  &  18 29 07.0 &  +00 30 41.5  &  1016 (14)  &  59.2  &  IRAS 18265+0028; MMS2 (2)  &  Y   \\
Bolo15  &  18 29 09.6 &  +00 31 36.9  &  626 (14)  &  33.0  &  MMS3 (2)  &  Y   \\
Bolo16  &  18 29 13.5 &  +00 32 12.6  &  175 (13)  &  5.8  &    &  N   \\
Bolo17  &  18 29 16.4 &  +00 18 15.4  &  82 (8)  &  6.7  &  IRAS 18267+0016  &  Y   \\
Bolo18  &  18 29 19.3 &  +00 33 29.1  &  104 (12)  &  6.0  &    &  N   \\
Bolo19  &  18 29 31.5 &  +00 26 49.3  &  279 (14)  &  14.8  &  MMS4 (2)  &  N   \\
Bolo20  &  18 29 31.9 &  +01 19 00.9  &  337 (13)  &  18.3  &    &  Y   \\
Bolo21  &  18 29 43.4 &  +00 36 25.2  &  129 (11)  &  7.7  &    &  N   \\
Bolo22  &  18 29 48.8 &  +01 16 50.6  &  1694 (16)  &  80.7  &  SMM 9 (1); S68N  &  Y   \\
Bolo23  &  18 29 50.2 &  +01 15 24.6  &  3010 (20)  &  138  &  SMM 1 (1); FIRS 1  &  Y   \\
Bolo24  &  18 29 53.8 &  +00 36 10.1  &  202 (10)  &  17.2  &  IRAS 18273+0034  &  Y   \\
Bolo25  &  18 29 57.4 &  +01 13 14.9  &  1980 (23)  &  62.7  &  SMM 4 (1)  &  Y   \\
Bolo26  &  18 29 59.2 &  +01 14 07.4  &  1331 (19)  &  43.0  &  SMM 3 (1) &  Y   \\
Bolo27  &  18 30 00.3 &  +01 10 37.8  &  425 (19)  &  14.5  &    &  Y   \\
Bolo28  &  18 30 00.7 &  +01 12 56.5  &  1266 (19)  &  34.3  &  SMM 2 (1)  &  Y   \\
Bolo29  &  18 30 01.0 &  +01 11 49.1  &  979 (19)  &  33.5  &  SMM 11 (1)  &  Y   \\
Bolo30  &  18 30 02.5 &  +01 15 24.5  &  319 (16)  &  11.3  &  SMM 8 (1) &  Y   \\
Bolo31  &  18 30 02.8 &  +01 08 38.3  &  214 (16)  &  10.0  &    &  Y   \\
Bolo32  &  18 30 05.7 &  +00 39 32.2  &  105 (12)  &  5.0  &    &  Y   \\
Bolo33  &  18 30 06.4 &  +00 42 37.0  &  126 (11)  &  8.3  &    &  Y   \\
Bolo34  &  18 30 08.2 &  +01 13 11.5  &  153 (11)  &  7.8  &    &  N   \\
Bolo35  &  18 30 14.7 &  +01 13 52.6  &  85 (11)  &  5.6  &    &  N   \\
\enddata
\tablecomments{Numbers in parentheses are $1\sigma$ errors.   The peak flux density is the peak value per beam in the $10\arcsec$ pixel$^{-1}$  unfiltered map (without the optimal filter applied).  The uncertainty in the peak flux density is the local  rms beam$^{-1}$ and does not include an additional 15\% systematic uncertainty from calibration uncertainties and residual errors after iterative mapping.  Other names listed are the most common identifications from the literature, and are not meant to be a complete list.  A 1.1~mm source is considered coincident with a MIPS source if the position is within $60\arcsec$ of a $24~\micron$ source from the c2d catalog \citep{harv07}.  References -- (1) \citet{ced93}; (2) \citet{djup06}}
\end{deluxetable}
\endinput


==> tab2.tex <==
\ProvidesFile{tab2.tex}
\begin{deluxetable}{lccccccccccl}
%\rotate{90}
\tabletypesize{\scriptsize}
\tablecolumns{12}
\tablewidth{0pc}
\tablecaption{Photometry and Core Properties \label{phottab}}
\tablehead{
\colhead{ID} &  \colhead{Flux($40\arcsec$)}  &  \colhead{Flux($80\arcsec$)}  &  \colhead{Flux($120\arcsec$)} & \colhead{Total Flux}  & \colhead{Mass (10K)}  & \colhead{Peak $A_V$} & \colhead{FWHM} & \colhead{FWHM}  & \colhead{PA} & \colhead{$\mean{n}$}  & \colhead{Morphology\tablenotemark{1}} \\ 
\colhead{} &  \colhead{(Jy)}  &  \colhead{(Jy)}  &  \colhead{(Jy)} & \colhead{(Jy)}  & \colhead{($M_{\sun}$)} & \colhead{(mag)} & \colhead{(minor,$\arcsec$)} & \colhead{(major,$\arcsec$)}  & \colhead{($\degr$)}  &\colhead{cm$^{-3}$} & \colhead{}
}
\startdata
Bolo1  &  0.137 (0.016)  &   \nodata   &   \nodata    &  0.25 (0.03)   &   0.65 (0.07)   & 8   &  52 (1.0)  &  62 (1.2)  &  55 (8)  &  1.0$\times10^5$   &  extended,elongated,weak  \\		 
Bolo2  &  0.282 (0.017)  &   \nodata   &   \nodata    &  0.51 (0.03)    &   1.34 (0.08)   & 17  &  51 (0.5)  &  63 (0.6)  &  -57 (4)  &  2.1$\times10^5$   &  multiple,extended,elongated  \\	 
Bolo3  &  0.324 (0.015)  &   \nodata   &   \nodata    &  0.382 (0.019)  &   1.00 (0.05)   & 19  &  43 (0.4)  &  55 (0.5)  &  -77 (3)  &  3.2$\times10^5$ &  multiple,extended,round  \\		 
Bolo4  &  0.226 (0.013)  &   \nodata   &   \nodata    &  0.28 (0.017)   &   0.73 (0.04)   & 12  &  43 (0.5)  &  55 (0.6)  &  49 (4)  &  2.2$\times10^5$   &  multiple,extended,elongated  \\	 
Bolo5  &  0.094 (0.013)  &   \nodata   &   \nodata    &  0.16 (0.02)    &   0.41 (0.06)   &  6  &  50 (1.2)  &  63 (1.4)  &  -68 (8)  &  7$\times10^4$    &  extended,round,weak  \\		 
Bolo6  &  0.172 (0.013)  &   \nodata   &   \nodata    &  0.210 (0.016)  &   0.55 (0.04)   & 10  &  46 (0.6)  &  62 (0.8)  &  -40 (3)  &  1.1$\times10^5$  &  multiple,extended,elongated  \\	 
Bolo7  &  0.162 (0.015)  &   \nodata   &   \nodata    &  0.162 (0.015)  &   0.42 (0.04)   & 10  &  46 (0.8)  &  57 (0.9)  &  -30 (7)  &  1.0$\times10^5$  &  multiple,extended,elongated  \\	 
Bolo8  &  0.933 (0.018)  &   1.99 (0.04)  &   \nodata    &  2.63 (0.04) &   6.87 (0.12)   & 52  &  62 (0.2)  &  74 (0.2)  &  68 (1)  &  5.2$\times10^5$   &  multiple,extended,round  \\		 
Bolo9  &  \nodata   &   \nodata   &   \nodata    &  0.169 (0.010)       &   0.44 (0.03)   & 12  &  38 (0.5)  &  61 (0.7)  &  -58 (2)  &  1.5$\times10^5$      &  multiple,extended,elongated  \\	 
Bolo10  &  0.146 (0.015)  &   \nodata   &   \nodata    &  0.146 (0.015) &   0.38 (0.04)   &  9  &  51 (0.8)  &  54 (0.9)  &  11 (25)  &  8$\times10^4$  &  multiple,extended,elongated  \\	 
Bolo11  &  \nodata   &   \nodata   &   \nodata    &  0.199 (0.011)      &   0.52 (0.03)   & 14  &  37 (0.4)  &  61 (0.7)  &  -59 (2)  &  1.8$\times10^5$     &  multiple,round,  \\	
Bolo12  &  0.246 (0.014)  &   \nodata   &   \nodata    &  0.246 (0.014) &   0.64 (0.04)   & 15  &  39 (0.4)  &  58 (0.6)  &  -65 (2)  &  2.2$\times10^5$ &  multiple,extended,elongated  \\	 
Bolo13  &  0.36 (0.02)  &   \nodata   &   \nodata    &  0.36 (0.02)     &   0.94 (0.05)   & 20  &  52 (0.5)  &  59 (0.5)  &  -78 (6)  &  1.7$\times10^5$   &  multiple,extended,round  \\		 
Bolo14  &  1.381 (0.019)  &   \nodata   &   \nodata    &  2.16 (0.03)   &   5.65 (0.09)   & 86   &  47 (0.1)  &  54 (0.1)  &  -44 (2)  &  1.5$\times10^6$   &  multiple,extended,elongated  \\	 
Bolo15  &  0.856 (0.018)  &   \nodata   &   \nodata    &  0.856 (0.018) &   2.24 (0.05)   & 53  &  44 (0.2)  &  56 (0.2)  &  -27 (1)  &  6.5$\times10^5$  &  multiple,extended,round  \\		 
Bolo16  &  0.222 (0.018)  &   \nodata   &   \nodata    &  0.27 (0.02)   &   0.71 (0.06)   & 15  &  42 (0.5)  &  62 (0.8)  &  32 (3)  &  1.8$\times10^5$   &   multiple,extended,elongated  \\	 
Bolo17  &  0.118 (0.011)  &   0.24 (0.02)  &  0.4 (0.03) &  0.40 (0.03) &   1.05 (0.09)   &  7  &  80 (1.1)  &  97 (1.3)  &  -66 (5)  &  3$\times10^4$ &  extended,elongated  \\		 
Bolo18  &  0.144 (0.016)  &   \nodata   &   \nodata    &  0.25 (0.03)   &   0.65 (0.08)   &  9  &  48 (0.8)  &  71 (1.2)  &  -41 (3)  &  9$\times10^4$   &  multiple,extended,elongated,weak  \\	 
Bolo19  &  0.41 (0.018)  &   0.85 (0.04)  &  1.28 (0.06) &  1.28 (0.06) &   3.34 (0.14)   & 24  &  74 (0.5)  &  89 (0.6)  &  -74 (3)  &  1.3$\times10^5$ &  extended,elongated  \\		 
Bolo20  &  0.494 (0.018)  &   1.01 (0.04) &  1.57 (0.05) &  1.57 (0.05) &   4.11 (0.14)   & 29  &  87 (0.5)  &  90 (0.5)  &  9 (11)  &  1.2$\times10^5$ &  extended,elongated  \\		 
Bolo21  &  0.177 (0.014)  &   0.38 (0.03)  &   \nodata   &  0.38 (0.03) &   0.98 (0.07)   & 11  &  53 (0.7)  &  64 (0.8)  &  47 (6)  &  1.3$\times10^5$ &  multiple,extended,elongated  \\	 
Bolo22  &  2.32 (0.02)  &   \nodata   &   \nodata    &  3.78 (0.04)     &   9.86 (0.10)   & 144  &  47 (0.1)  &  57 (0.1)  &  73 (1)  &  2.3$\times10^6$    &  multiple,extended,round  \\		 
Bolo23  &  3.8 (0.03)  &   5.91 (0.05)  &   \nodata    &  5.91 (0.05)   &   15.44 (0.14)  & 256  &  46 (0.1)  &  47 (0.1)  &  39 (4)  &  6.1$\times10^6$    &  multiple,extended,round  \\		 
Bolo24  &  0.291 (0.014)  &   \nodata   &   \nodata    &  0.40 (0.02)   &   1.04 (0.05)   & 17  &  46 (0.4)  &  55 (0.5)  &  -12 (4)  &  2.9$\times10^5$   &  multiple,extended,elongated  \\	 
Bolo25  &  2.75 (0.03)  &   \nodata   &   \nodata    &  3.19 (0.04)     &   8.33 (0.10)   & 168  &  44 (0.1)  &  51 (0.1)  &  79 (1)  &  2.9$\times10^6$    &  multiple,extended,round  \\		 
Bolo26  &  1.9 (0.03)  &   \nodata   &   \nodata    &  1.90 (0.03)      &   4.95 (0.07)   & 113  &  48 (0.1)  &  59 (0.1)  &  -21 (1)  &  1.0$\times10^6$   &  multiple,extended,round  \\		 
Bolo27  &  0.65 (0.03)  &   \nodata   &   \nodata    &  1.18 (0.05)     &   3.09 (0.12)   & 36  &  47 (0.3)  &  69 (0.4)  &  89 (1)  &  4.6$\times10^5$   &    multiple,extended,elongated  \\	 
Bolo28  &  1.9 (0.03)  &   \nodata   &   \nodata    &  1.90 (0.03)      &   4.96 (0.06)   & 108  &  48 (0.1)  &  59 (0.1)  &  -47 (1)  &  1.0$\times10^6$   &   multiple,extended,round  \\		 
Bolo29  &  1.41 (0.03)  &   \nodata   &   \nodata    &  2.44 (0.05)     &   6.37 (0.12)   & 83   &  47 (0.1)  &  59 (0.2)  &  -86 (1)  &  1.4$\times10^6$   &   multiple,extended,round  \\		 
Bolo30  &  0.43 (0.02)  &   \nodata   &   \nodata    &  0.43 (0.02)     &   1.13 (0.06)   & 27  &  48 (0.4)  &  55 (0.5)  &  33 (5)  &  2.6$\times10^5$   &    multiple,extended,elongated  \\	 
Bolo31  &  0.32 (0.02)  &   0.65 (0.04)  &   \nodata    &  0.65 (0.04)  &   1.70 (0.11)   & 18  &  45 (0.5)  &  74 (0.8)  &  -65 (2)  &  2.4$\times10^5$  &  multiple,extended,elongated  \\	 
Bolo32  &  0.151 (0.016)  &   0.34 (0.03)  &   \nodata  &  0.34 (0.03)  &   0.88 (0.08)   &  9  &  57 (0.9)  &  74 (1.2)  &  50 (5)  &  8$\times10^4$ &  extended,elongated  \\		 
Bolo33  &  0.12 (0.015)  &   \nodata   &   \nodata    &  0.128 (0.019)  &   0.34 (0.05)   & 11  &  35 (0.9)  &  39 (1.1)  &  25 (17)  &  6.9$\times10^6$  &  round  \\				 
Bolo34  &  0.181 (0.015)  &   \nodata   &   \nodata    &  0.216 (0.019) &   0.56 (0.05)   & 13  &  40 (0.6)  &  60 (0.9)  &  -70 (3)  &  1.7$\times10^5$  &  multiple,extended,elongated  \\	 
Bolo35  &  \nodata   &   \nodata   &   \nodata    &  0.06 (0.011)   &   0.16 (0.03)       &  7  &  24 (1.1)  &  61 (2.9)  &  -69 (4)  &  2.4$\times10^5$  &  multiple,weak  \\                  
\enddata
\tablecomments{Masses are calculated according to Eq.~\ref{masseq} from the total flux density assuming a single dust temperature of $T_D=10$~K and a dust opacity at 1.1mm of $\kappa_{1.1mm} = 0.0114$~cm$^2$g$^{-1}$.  Peak $A_V$ is calculated from the peak flux density as in Eq.~\ref{aveq}.  FWHM and PAs are from an elliptical gaussian fit; the PA of the major axis is measured in degrees east of north.  $\mean{n}$ is the mean particle density as calculated from the total mass and the deconvolved average FWHM size.  Numbers in parentheses are $1\sigma$ uncertainties.  Uncertainties for masses are from photometry only, and do not include uncertainties from $\kappa$, $T_D$, or $d$, which can be up to a factor of a few or more.  Uncertainties for the FWHM and PA are formal fitting errors from the elliptical gaussian fit; additional uncertainties of $10-15$\% apply to the FWHM, and $\sim5\degr$ to the PA (determined from simulations).}
\tablenotetext{1}{The morphology keywords given indicates whether the source is multiple (within $3\arcmin$ of another source), extended (major axis FW at $2\sigma > 1\arcmin$), elongated (axis ratio at $4\sigma > 1.2$), round (axis ratio at $4\sigma < 1.2$), or weak (peak flux density less than 5 times the rms pixel$^{-1}$ in the unfiltered map).}
\end{deluxetable}
\endinput


==> tab3.tex <==
\ProvidesFile{tab3.tex}
\begin{deluxetable}{lcccccc}
%\rotate
\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{Cumulative Mass as a Function of Extinction \label{avtab}}
\tablehead{
\colhead{Min. $A_V$}
& \colhead{Area}
& \colhead{Cloud Mass}
& \colhead{Percent}
& \colhead{Core Mass}
& \colhead{Percent}
& \colhead{Mass Ratio\tablenotemark{1}}  \\
\colhead{mag}
&  \colhead{(\%)}
&  \colhead{(\msun)}
&  \colhead{(\%)}
&  \colhead{(\msun)}
&  \colhead{(\%)}
&  \colhead{(\%)}
}
\startdata
\cutinhead{Serpens}
\ 2	&  100	& 3470	&  100 	& 92	& 100   &  2.7 	  \\
\ 4	&  97	& 3420	&  99	& 92	& 100 	&  2.7	  \\
\ 6	&  60	& 2560	&  74	& 92	& 100	&  3.6	  \\
\ 8	&  28	& 1530	&  44	& 91	&  98	&  5.9	  \\
10	&  15	& 1010	&  29	& 91	&  98	&  9.0	  \\
12	&  9.4	& 740	&  21	& 89	&  96	&  12	  \\
14	&  6.0	& 540	&  15	& 89	&  96	&  16	  \\
16	&  3.9	& 390	&  11	& 86	&  93	&  22	  \\
18	&  2.6	& 290	&  8.3	& 83	&  90	&  29	  \\
20	&  2.0	& 230	&  6.7	& 79	&  85	&  34	  \\
25	&  1.0	& 130	&  3.7	& 61	&  66	&  47	  \\
30	&  0.4	& 60	&  1.7	& 39	&  42	&  65	  \\
%35	&  0.1	& 15	&  0.4	& 17	&  19	&  110	  \\
\cutinhead{Perseus}
\ 2	&   100	&  7340	&  100 	& 278	& 97   &  3.8	  \\
\ 4	&   55	&  5460	&  74	& 273	& 96 	&  5.0	  \\
\ 6	&   27	&  3620	&  49	& 258	& 91 	&  7.1	  \\
\ 8	&   14	&  2370	&  32	& 244	&  86	&  10	  \\
10	&   8.0	&  1620	&  22	& 205	&  72	&  13	  \\
12	&   4.8	&  1140	&  15	& 161	&  57	&  14	  \\
14	&   3.2	&  840	&  12	& 127	&  45	&  15	  \\
16	&  2.0	& 610	&  8.3	& 112	&  39	&  18	  \\
18	&  1.3	& 440	&  6.0	& 96	&  34	&  22	  \\
20	&  0.9	& 340	&  4.6	& 88	&  31	&  26	  \\
25	&  0.4	& 180	&  2.5	& 53	&  19	&  29	  \\
30	&  0.2	& 100	&  1.4	& 6.1	&  2.2	&  6.1	  \\
%35	&  0.1	& 58	&  0.8	& 5.3	&  1.8	&  9.1	  \\
\cutinhead{Ophiuchus}
\ 2	& 100	& 3570	& 100	& 44	& 100   & 1.2	  \\
\ 4	& 55	& 2710	& 76	& 44	& 100	& 1.6	  \\
\ 6	& 25	& 1830	& 51	& 40	& 92	& 2.2 	  \\
\ 8	& 14	& 1330	& 37	& 40	&  92	& 3.0	  \\
10	& 9.0	& 1070	& 30	& 40	&  92	& 3.7 	  \\
12	& 7.0	& 940	& 26	& 40	&  92	& 4.3 	  \\
14	& 5.6	& 820	& 23	& 40	&  92	& 4.9 	  \\
16	& 4.6	& 730	& 20	& 40	&  92	& 5.5 	  \\
18	& 3.8	& 640	& 18	& 39 	&  90	& 6.1 	  \\
20	& 3.1	& 560	& 16	& 37	&  84	& 6.6	  \\
25	& 2.0	& 400	& 11	& 32	&  73	& 8.0	 \\
30	& 1.2	&  260	& 7.3	& 23	&  52	& 8.8	 \\
%35	& 0.6	&  150	& 4.3	& 7.0	&  16	& 4.7	 \\
\enddata
\tablecomments{
Cloud areas and masses are calculated using the c2d extinction maps 
(see \S~\ref{ressect}) of each 
cloud and Eq.~\ref{avmasseq}.  Core masses are taken from Table \ref{phottab}.
}
\tablenotetext{1}{The Mass Ratio is computed from the ratio of total core mass to
cloud mass within the same contour of \av.}
\end{deluxetable}
\endinput

